The Maximal Subword Complexity of Quasiperiodic Infinite Words

We provide an exact estimate on the maximal subword complexity for quasiperiodic infinite words. To this end we give a representation of the set of finite and of infinite words having a certain quasiperiod q via a finite language derived from q. It is shown that this language is a suffix code having a bounded delay of decipherability. Our estimate of the subword complexity now follows from this result, previously known results on the subword complexity and elementary results on formal power series.

==> eptcsdata.tex <==
\providecommand{\firstpage}{169}
\providecommand{\publicationstatus}{I. McQuillan and G. Pighizzini (Eds.): 12th International Workshop\\on Descriptional Complexity of Formal Systems (DCFS 2010)\\
EPTCS 31, 2010, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.31.19}{10.4204/EPTCS.31.19}}

